Finding Trends in Software Research

This paper explores the structure of research papers in software engineering. Using text mining, we study 35,391 software engineering (SE) papers from 34 leading SE venues over the last 25 years. These venues were divided, nearly evenly, between conferences and journals. An important aspect of this analysis is that it is fully automated and repeatable. To achieve that automation, we used a stable topic modeling technique called LDADE that fully automates parameter tuning in LDA. Using LDADE, we mine 11 topics that represent much of the structure of contemporary SE. The 11 topics presented here should not be "set in stone" as the only topics worthy of study in SE. Rather our goal is to report that (a) text mining methods can detect large scale trends within our community; (b) those topic change with time; so (c) it is important to have automatic agents that can update our understanding of our community whenever new data arrives.

==> dependencies.tex <==
\RequirePackage{xcolor}
\ifCLASSOPTIONcompsoc
  % The IEEE Computer Society needs nocompress option
  % requires cite.sty v4.0 or later (November 2003)
  \usepackage[nocompress]{cite}
\else
  % normal IEEE
  \usepackage{cite}
\fi
\usepackage{array}
\usepackage{lineno,hyperref}
\usepackage{multirow}
\usepackage{setspace}
\usepackage{balance}
\usepackage{flushend}
% \usepackage{natbib}
\usepackage{color} 
\usepackage{graphics} 
% \usepackage{cite}
\usepackage{rotating}
\usepackage{eqparbox}
\usepackage{graphics}
\usepackage{colortbl}
\usepackage{wrapfig}
\usepackage{times}
%\usepackage{mathptmx} \usepackage[scaled=.90]{helvet} \usepackage{courier}
% \usepackage{balance}
\usepackage{flushend}
\usepackage{picture}
\usepackage{algorithm}
\usepackage{algorithmicx}
\usepackage{algpseudocode}
\usepackage[export]{adjustbox}
\usepackage{amsmath}
\usepackage{listings}
\usepackage{mdframed}
\usepackage{algorithm,algorithmicx}
\usepackage{algpseudocode}
\usepackage{wrapfig}
\usepackage{caption}

\usepackage{rotating}
\definecolor{Gray}{rgb}{0.88,1,1}
\definecolor{Gray}{gray}{0.85}
\definecolor{Blue}{RGB}{0,29,193}
\definecolor{rc1}{RGB}{253,237,236}
\definecolor{rc2}{RGB}{218,247,166}
\definecolor{rc3}{RGB}{174,214,241}
\definecolor{rc4}{RGB}{242,244,244}
\definecolor{rc5}{RGB}{255,195,0}
\definecolor{rc6}{RGB}{199,0,57}
\definecolor{rc7}{RGB}{144,12,63}
\definecolor{plotBlue}{RGB}{4,51,255}
\definecolor{plotRed}{RGB}{255,38,0}

\renewcommand{\footnotesize}{\scriptsize}
\definecolor{lightgray}{gray}{0.8}
\definecolor{darkgray}{gray}{0.6}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
%%% graph
\newcommand{\crule}[3][darkgray]{\textcolor{#1}{\rule{#2}{#3}}}
\definecolor{Gray}{gray}{0.95}
\definecolor{LightGray}{gray}{0.975}

%% timm tricks
\newcommand{\eref}[1]{Eq.~\ref{eq:#1}}
\newcommand{\fref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tref}[1]{Table~\ref{tab:#1}}
\newcommand{\boldm}[1]{$\bm{#1}$}
\newcommand{\bit}[1]{\textbf{\textit{#1}}}
\newcommand{\bi}{\begin{itemize}[leftmargin=0.4cm]}
\newcommand{\ei}{\end{itemize}}
\newcommand{\be}{\begin{enumerate}}
\newcommand{\ee}{\end{enumerate}}
\newcommand{\tion}[1]{Section \ref{sect:#1}}
\newcommand{\fig}[1]{Figure~\ref{fig:#1}}
\newcommand{\tab}[1]{Table~\ref{tab:#1}}
\newcommand{\eq}[1]{Equation~\ref{eq:#1}}
\newcommand{\PM}{$\pm$}
\newcommand{\desc}[1] {
    \medskip
    \raggedright
    \small
    #1
}
\newcommand{\bcell}[2][c]{%
  \begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}
\newcommand{\etal}{et al. }
%% space saving measures
\let\labelindent\relax
\usepackage[shortlabels]{enumitem}  
\usepackage{url}

\usepackage{graphicx}
\usepackage{multirow}
% \usepackage[svgnames]{xcolor}
% \usepackage[table, svgnames]{xcolor}
\usepackage[framed]{ntheorem}
\usepackage{framed}
\usepackage{tikz}
\usetikzlibrary{shadows}
%\newtheorem{Lesson}{Lesson}
\theoremclass{Lesson}
\theoremstyle{break}

% inner sep=10pt,
\tikzstyle{thmbox} = [rectangle, rounded corners, draw=black,
  fill=Gray!20,  drop shadow={fill=black, opacity=1}]
\newcommand\thmbox[1]{%
  \noindent\begin{tikzpicture}%
  \node [thmbox] (box){%
\begin{minipage}{.9\textwidth}%    
      \vspace{-3mm}#1\vspace{-3mm}%
    \end{minipage}%
  };%
  \end{tikzpicture}}

\let\theoremframecommand\thmbox
\newshadedtheorem{lesson}{Result}

\usepackage{array}
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

\newcommand{\mc}[2]{\multicolumn{#1}{|c|}{#2}}
\newcommand{\h}{\hspace{17pt}}
\newcommand{\hh}{\hspace{35pt}}
\newcommand{\rA}{\cellcolor{rc1}}
\newcommand{\rB}{\cellcolor{rc2}}
\newcommand{\rC}{\cellcolor{rc3}}
\newcommand{\rD}{\cellcolor{rc4}}
\newcommand{\rE}{\cellcolor{rc5}}
\newcommand{\rF}{\cellcolor{rc6}}
\newcommand{\legend}[2]{\colorbox{#1}{\makebox(9,3){}} #2}


==> replies.tex <==
%% Replies.pdf

\clearpage
\pagenumbering{roman}
\setcounter{page}{1}

\nobalance
\pagestyle{plain} 

\section*{Responses to reviewers}

Thank you for the opportunity to resubmit this work.
Thank you also for the extensive comments-- they were
very useful in clarifying and improving the previous draft.

Please see our replies to reviewer comments below. Note that anything in {\em italics} is from the review team. \\

\noindent
\textit{Comment from Editor: The most notable concerns are:}

\bi
\item \textit{R1 and R2 are concerned about the use of unpublished approach by the authors and cast doubts many of the used decisions in filtering out the output. More concretely they are doubtful of the need of the LDA variant over a basic LDA run.\\}

We thank the reviewers for pointing out those concerns. We have explained our reasoning of choosing a variant of LDA in Section~\ref{sect:ldade}. \\

\item \textit{R2 and R3 share concerns about many of the proposed recommendations. In particular, they felt that many of the results are poorly interpreted and feel a bit too much speculative in nature.\\}

We agree-- the last version's claims were far too grandiose. Based on reviewers feedback, this version is.... humbler.\\

\item \textit{As I read through their feedback, one thing that emerges is you are likely never going to be able to show the generality of the findings (there will always be a venue that is missing) and the interpretation of the results needs to be done quite carefully. Hence, you might want to reconsider the contribution of the work as a proposal for a general methodology that would be of value to anyone to feeding their venues of interest -- something that is already possible due to the availability of the tooling.\\}

We agree with you on this point.
Hence in this  draft we have made many changes
stressing that this paper is ``a'' method,
not ``the'' method, for finding   trends in SE
(for example, (a)~see our new title; (b)~see how
we have removed numerous overly-ambitious conclusions from
the previous version).\\

% \item \textit{I would then propose a more deeper investigation of some of the findings for particular sub-communities (e.g., contacting experts within these communities or whatever approach that authors feel is appropriate) instead of trying to fully interpret everything in a speculative manner. Please consider this as simply a suggestion instead of the only way to go about reworking the work.\\}
\ei


\section*{A. Reviewer 1}

\textit{For the most part, this paper seems to be an excellent contribution. The introduction, motivation, related work, data gathering, results, etc. all seem exemplary. And I feel it is an important paper that should be published as a resource for the community as a whole. It is clearly written, if a bit terse.\\}

Thank you for your kind words.\\

\textit{A.1.)  However they make a big deal in section 2.1.2 about Differential Evolution (a evolutionary method) to perform hyperparameter tuning. Although using GAs/search to perform LDA hyperparameter tuning has precedent in the SE literature it's still unnecessary and bizzare: the original LDA paper suggests how to do variational inference on the hyperparameters, and in fact this is implemented in off-the-shelf LDA packages such as gensim. The use of search to tune hyperparameters that can be estimated directly from the data while the rest of the model is being estimated is unnecessary and overly complicated, relying on work that has not been peer-reviewed as well. The citation is currently the author's own work on arXiv.  For tuning k, it is reasonable to perform a search, but not for tuning alpha or beta; Both alpha and beta can be estimated using gibbs or variational methods (as the authors themselves point out in their arXiv paper).\\}

The recent paper from Agrawal et al.~\cite{agrawal2016wrong} which is now published at Information and Software Journal shows the difference between their work and LDA-GA~\cite{panichella2013effectively} work. They came to a conclusion that some of LDA-GA's drawbacks are overcome by LDADE. Also, we agree  with you that the   original LDA paper~\cite{blei2003latent} estimates alpha, and beta while updating the model. However, we also note
that in   the literature there are now several
papers reporting that it is better to use
other methods to find those parameter~\cite{panichella2013effectively,lohar2013improving,agrawal2016wrong}.
 
~\\

\textit{A.2. The authors chose to use ``raw score'' (their own invention) as a metric of goodness of the model when LDA is a (produces a) generative Bayesian model and the likelihood of the model given the data can be estimated as per the original LDA paper. Their raw score measures topic stability, which is between two independent runs of LDA, how similar the topics are. (This is not described in this paper, it is only described in the unreviewed citation on arXiv by the authors.) However there is no reason that is the best metric for LDA in this paper, and simply choosing relatively large values for alpha and beta and a relatively small k will always yield more stable (in their definition, not in this paper) topics, because of the very nature of the hyper-parameters themselves. In other words, it's easier to get two pictures taken one after another to look the same if you apply a blur to them both!\\}

LDADE work (now published in Information and Software Technology journal) have shown the generated topics from LDA generated from SE papers are highly unstable~\cite{agrawal2016wrong}. We ran their LDADE  experiments to show whether the stability in this work matters as well (see \fref{topic_overlaps}). Please note in that figure, we observed that the LDADE generated more stable topics than standard LDA.
Therefore we believe that LDADE is a significant value added for this work.\\

\textit{A.3. I would argue that the best metric of fitness for the model in this paper is how well the inferred model (and therefore topics) matches the data. However, if stability is desired, it is always possible to initialize the LDA parameters (not the hyperparameters) based on the previous run of LDA. This functionality is also available in off-the-shelf LDA packages.\\}

As per your suggestion we ran LDA after initializing the parameters based on the engineering judgement and used LDADE to automatically find the right hyperparameters. Please see figure~\ref{fig:naive_vs_ldade} where we can see the right cut-off for number of topics came out to be 11 with LDADE and 20 with LDA.

That is:
\bi
\item The method you suggested above is certain simpler and faster;
\item However, when we conduct a more extensive analysis of the domain (using LDADE), we find different and better topics.
Specifically, in \fref{naive_vs_ldade}, we see the blue line (from LDADE) peak peeks to a higher point than the red line (using your method, which in turn, used the settings from Blei et al, 2003).
The difference is small, but significantly, we can achieve the superior blue peek using nearly half the topics of the red line.
\item For these reasons, we still argue that LDADE is a significant value added component of this work.\\
\ei

\textit{A.4. Section 2.1.2 should be removed and the experiments should be re-run with standard hyperparameters or by using variational inference to estimate the hyperparameters from the data as described by Blei et al, 2003, in the original LDA paper.  I should note that, once this is done, I do not expect the results to change significantly.\\}

We understand why you are making that recommendation-- but given our recent IST publication and the experiments reported above, our view is that  our LDADE is a significant value-added component of this week. 

But we mean no disrespect to your suggestions. Please note that we did do as you suggested (used the default Blei et al results in section \ref{sect:ldade})
so we did try your approach. But the \fref{topic_overlaps} results are very clear: with LDADE we can achieve stabler results using a much less complex
model (using 11 topics, not 20)..

Please also see our replies to A.2 and A.3. We show that LDADE results are more stable and k=11 topics is a good choice.\\

\textit{A.5. The authors should also discuss in their threats to validity the fact that k=11 is essentially arbitrary (even if it does minimize their invented metric) and there may be more or less than 11 discrete topics in the literature if users were surveyed. Similarly, the authors make a fair argument by spot checking the topics that the topics are in fact correct, but of course the authors are biased toward reaching this decision and its impossible to conclude that they are without surveying SE practitioners.\\}

Please see our reply to A.3 and section~\ref{sect:topicSanity}. We do agree that surveying SE practitioners will provide better validity and that is why we formulated this paper as a mean to find trends in software research.\\

\textit{A.5. I should note, however, that this does does not invalidate the contribution of the paper as a whole, which, seems important and valuable to the community. It only means that some topics are probably too big, overlapping too much with the other topics, and some may be merged. The results of this paper are still valuable but they must be framed in a way that does not claim these topics are The True Eleven Topics of SE, this is merely a useful clustering not the true clustering. One would imagine even two different SE researchers would disagree on the number and organization of topics in the conferences and journals studied.\\}

We agree and disagree with your comment. Firstly, we agree that some trite statement of ``The Elven Topics of SE'' would be a ridiculous and detrimental summary of this work. To stress your point,
we have added the following text 
to the conclusion and our abstract:

\begin{quote}
... it must be stressed
that the 11 topics presented here
should not be ``set in stone''
as the only  topics   worthy of study in SE.
Rather it is to report that   (a)~text mining methods can  detect large scale trends within our community;  (b)~those topics
 change with time; so (c)~it is  important to have automatic agents that can update our understanding
of our community
whenever new data arrives. An important feature of such agents is that
they must be  {\em trustworthy}. What we show here is that the LDADE method (described
below) is a significant contributor 
to topic stability and hence the trustworthiness of this analysis. 
\end{quote}

Secondly, we disagree that these 11 topics are an arbitrary construct. In fact, you may be surprised at how stable are our 11 topics.We have expanded our corpora  twice (once in early 2017, once later that year) and in both expansions, essentially the same structures
were present before and afterwards. This paper even  offers one example of those stability.  In section~\ref{sect:topicAdapt} we show that when a chunk of the venues are removed, the majority of the clusters remain same and stable. Thus, this technique although useful can produce a good estimate of the true clusters in SE if provided with a large set of papers from a diverse set of venues.




\section*{B. Reviewer 2}

\textit{The authors produce a very valuable piece of research that may spearhead the innovation which IMHO is much direly needed across our research community, especially considering several late events that showed a community in disarray rather than a solid, established social structure. That being said, I commend the authors for their work but found at least two major shortcomings that deserve their attention.\\}

Thank you for your support.\\

\textit{B.1. First, the results are indeed extremely needed and impactful.\\}

Yet again, thank you for endorsing the impact of this study. \\

\textit{B.1
... but I fear that the selection of venues, and journals may be lacking some qualitative confirmation. More in particular, for example, I was intrigued to observe that, while several topics reflect certain very specific and also reasonably impactful venues (e.g., ICPE for performance, or WICSA/ICSA for Architectures) these were not selected for the sample set under inquiry. This is a major problem since it cannot warrant publication of the results and the arguments produced (e.g., how would fig. 6 change by adding papers from ICPE and WICSA/ICSA?). I think the authors should make an effort to be able to address this point in a major revision, since I would really like to see this work published.\\}


The venues chosen in this study were based on a) suggestions from multiple previous submissions, b) rankings on google scholar and c) availability of the data from the venues. 

Now as to your suggestion of including ICPE and ICSA, we have some ungood  news and some much better news.

The ungood news is that these venues are not crawlable at this time (we mean no disrespect to those venues-- it is only recent that most conferences even acknowledge the need from crawling; e.g. the  IST journal was not crawlable up until very recently  in mid-2017).

The good news is that we have had the experience of expanding our corpora several times over the development of this week.
We find that as we add more and more venues, our clusters and topics are changing less and less. As evidence of this,
in this latest draft, we did do a study where we DELETED our   most recent venues (MODELS, SCAM, ICPC, SOSYM) and compared the learned
structures before and after that deletion. Essentially there was no change suggesting that further additions might have limited impact on the established structure.

For full details on that study, please see~\ref{sect:topicSanity}.\\


\textit{B.2. Second, many of the results and at least two of the recommendations are either banale, in progress (e.g., conference merging is a pretty big organizational topic as of late, not only in the software engineering backyard) or somewhat diminishing of the content and material available to the authors (e.g., merging Journals is a publisher decision, therefore it cannot be seen as a recommendation for the general software engineering public, while the present journal is). A similar comment may apply to journals as well.\\}

Thank you. We agree with you completely. Those sections are now  removed from the current work.\\

\textit{B.2 (more):
In summary, I think the practical and actionable RQs of this study deserve some attention in terms of offering insights over how the community leaders can and should shepherd their own communities towards more promoting, better collaborating ecosystem.\\}

We agree with you that the important aspect of this paper is its {\em practical implications}. To this end, this paper has conducted several case
studies to better understand aspects of our community. Specifically, the following items are now highlighted in the introduction and list
of contributions (see page1). 

\bi
\item Impact of generalist or specialist publishing habits (section \ref{sect:study_jack}). Based on that study, we conclude that
our community rewards ``breadth'' (exploring many topics) over ``depth'' (exploration of a small number of topics). Hence we would
encourage junior faculty to strive more to be polyglots rather than manically focus on just one small area.
\item Presence of Gender Bias in SE research (section \ref{sect:study_bias}). This result addressed an alarming possibility-- that women are
being  systematically  excluded from influential positions in SE. To our relief, we found that the percent of women on PCs is the same as the general research population. Which means that there is nothing earth shattering to report here. However, our point is that the tools,
data, and methods of this paper can be used to check important aspects of our field.
\item What is the  hottest topics in SE research (section \ref{sect:study_hot}). Our time series analysis shows that ``hottest topic''
is a dynamic concept. Topics like Source Code, Program Analysis and Testing have become popular over the last decade but topics like Performance and Security have become more scarce. This snapshot of trends in hottest topics would help a) funding bodies, b) editors of software journals and c) organizers of conferences to steer their research
\item Comparing and contrasting conferences and journals (section \ref{sect:study_conf_vs_jour}). 
From \tref{venue_vs_cites} we show that, until very recently, conferences and journals swapped round which kind of venue earned the most citations.
Now, in the last four years, the trend has changed: conferences now earn more citations than journals. Going forward,
this would be an important aspect of the SE publication model that, say, junior colleagues should keep in mind.\\
\ei

\textit{B.2 (more)
The most closely related RQ Questions such as ``Which topic is typically addressed in which conference/journal?'' should ensue from a study such as this, since, if the authors were to reveal that the top-conference in software engineering doesn't address all topics as broadly as it should then it *shouldn't* be considered the top conference in software engineering - the recommendation here would be that conference managers rethink their role as community leaders and reshape the actual goal of the conference, perhaps broadening or even diminishing its scope rather than ``claiming'' it is in fact a general purpose venue.\\}

Thank you for the text of the above recommendation. We have added that to the text (see section \tion{study_hot}).

At your suggestion, we checked for exactly that effect. 
Please see end of section 5.1. Here we assess the ``generalist'' nature of our big conference (ASE, ICSE, FSE, SANER) and journals
(TSE, TOSEM). The outstanding feature of our results is that that for these ``generalists'' venues, they have far fewer concentrations
of topics than the other, more specialist venues. The inclusion of ASE in that set might seem surprising. However,
as Micheal Whalen (personnel communication) said at a recent ASE meeting,
when the conference began, very little SE was automated. But now, in the age of DevOps and pipeline tool support, most of SE includes at some aspects of automation.

Hence, we say that our approach {\em can} test for conferences that claim to be ``general'' but, in fact, are not.\\

\textit{B2. (more)
To this dire point is RQ4 - perhaps the authors can explode that RQ with conference and journal specific gaps whose analysis can be elaborated using time-series analysis as well, to offer a quantitative perspective.\\}

We tried some time series work (ARIMA, moving averages, etc) but the general rule of thumb in that area is ``30 points or more''-- see \url{https://robjhyndman.com/hyndsight/short-time-series/}. So our 25 years is too short for standard time series methods.

 
 
That said, while we cannot exactly follow your suggestion,
we can do something like it (assess temporal patterns in different kinds of venues). For example, we have shown our contrasting results  between journals and conferences in section~\ref{sect:study_conf_vs_jour}.\\
 
 \textit{B.3. Similarly, based on the authors insights, perhaps a valuable recommendation could become that of creating a federated conference along the lines and findings of this study. There are those in our community who would not see it in any different shape than it is today, and in that case, rather than merging (which is admittedly a long and strenuous process, by direct experience) they may still welcome a schema wherefore multiple events *always* co-locate, co-operate, communicate, collaborate following an open-world organizational structure rather than one exhibiting a rigid-thinking establishment.\\}

This is an interesting observation but the current version of this paper now addresses the method in finding trends in software research. Hence this suggestion might not be suitable with the current direction of this paper. But based on your suggestion we are planning on an extension which can explore such applications of this method.  \\


 \textit{B.4. minor comments:
-(... numerous editorial suggestions\\}

Thank you. We fixed all the points your raised.\\

\textit{(B.4 More):
- Fig.s 5 and 6: as much as I like stacked diagrams they use colouring schemas which may inhibit certain readership, for example, I printed the paper B/W and had to reprint it, please consider using a different format... also, for some reason the elaboration of the results is somewhat counter intuitive (less frequent topics on the top) - consider revisiting these two figures;\\}

At your request, we made several attempts to alter that figure (e.g. lines, sequential bar charts, etc). We have to report that compared
to everything else we tried, the current figure displayed
the effects in the clearest manner.\\

\textit{B4 (more)
- Fig. 7   this figure is not really useful since you can elicit results and visualizations similar to it from several tools and overviews already available online... please provide some rationale as to why the fig. is useful or some interpretation as to its originally intended sense;\\}

Thank you for pointing this out. We agree to this and is now summarized in \tref{venue_vs_cites}.\\

\textit{B4 (more)
- Table 5: there seems to be a bit of theory behind the interpretation of this table and the results coded there-in but that theory is obscure to me... what was the original conjecture for determining this table and what is the recommendation after generating it? What I can gather from the table is that we do not have a clear identity of how to use a venue such as a conference and how to address a mature research result in a journal; with respect to this point, I see here no discussion, no research question, nor elaboration; there really should be some more discussion over this since it seems a valuable learning point and a key finding of the study;\\}

Thank you for letting us know about the missed theory in the previous table 5. We have now simplified it to just contain the median and IQR for the average number of citations per year for conferences and journals in \tref{venue_vs_cites}. On a high level it seems that conferences have become more popular over the last 4 years but when we delve much deeper into the table and \fref{topic_evo_conferences} and \fref{topic_evo_journals}, we can make some observations and recommendations.

\bi
\item The rising popularity of conferences might force upcoming researchers to publish in conferences over journals. This is a troubling trend for editors of journals and should be addressed by them.
\item If a researcher's concentration is on metrics, modelling or requirements, they should try to publish it in a journal as there are higher number of publications for these topics in journals.
\item Conversely, for topics like testing, program analysis and source code, researchers should try to publish it in conferences.\\
\ei
 
 \textit{B4 (more):
- Sec. 7: as much as I appreciate your politically-correctness in using ``some'' rather than explicit recommendations targeted explicitly to conference managers, I really think the recommendations should be lowered in terms of their level of abstraction, instantiating explicitly which conference should merge and why, i.e., stemming from which analysis, data points, etc. - also in relation to my major comment \#2\\}


There was some feedback from the Associate Editor suggesting that this section was a bridge too far. Hence, we have removed that material.\\


\textit{I really think this is the major contribution of this article and I cannot recommend for acceptance until these explicit and data-driven recommendations can be made explicit.\\}

At your recommendation, we have explored such data-driven conclusions. The new introduction highlights those on page1 and in the list of contributions.\\


\section*{C. Reviewer 3}

\textit{C.1. First of all, I did like the design and machinery used for the study. In particular, the advantages of LDADE seem legit for this study, and the combination with topical clustering allows automated abstraction in the large search space formed by thousands of papers. That said, more details are needed about the distance used for clustering (just based on topic distribution?).\\}

Thank you for the kind words. We now describe the complete linkage based hierarchical clustering scheme used in our technique in Section \ref{sect:clusters}. \\


\textit{C.1(more). Furthermore, I would like to see a comparison with results obtained using regular LDA, if one would estimate the topics manually (using existing heuristics). Is LDADE really essential?\\}

Based on your feedback we ran LDA after initializing the parameters based on the engineering judgement and used LDADE to automatically find the right hyperparameters. In \fref{naive_vs_ldade} where we can see the right cut-off for number of topics came out to be 11 with LDADE and 20 with LDA. Further, we turn your attention to \fref{topic_overlaps} which shows the percentage of common terms on different input ordering of the documents. We can see that LDADE is much more stable compared to LDA. Although the time taken for building the model is more expensive it is a one time process which yields a more stable model and better representation of documents. For greater detail on the study we point you to section \ref{sect:ldade}.\\



\textit{C.2. I wonder to what degree 11 topics can really capture the variance present in 35k papers. Although that low number enables the reader to grasp the results, it does not allow for substantial nuances in the way conferences are categorized. For example, MSR indeed considers source code analysis and developers, but its main focus is more generic on techniques for mining software repositories for a variety of sub problems, while other conferences like SCAM focus on static analysis for source code by itself. Also, the position of SANER away from WCRE/CSMR/ICSME seems different from what personal experience shows. A domain like real-time software is merged into OOPS, while the performance of systems is merged with the performance of algorithms.\\}

This is an interesting point you bring up. We agree that 11 topics may not be sufficient to capture the variance in all of software engineering particularly substantial nuances and niche domains. As you have pointed out there are a few exceptions to this study. These can be pointed out to
\bi
    \item Firstly, we consider only abstracts and titles in this proposed method due to its availability. The abstracts and titles generally summarizes the problem, the solution and results without delving into the technical details of each paper.
    \item Secondly, the number of samples for each topic in this study is different primarily due to the intrinsic nature of research. All topics in research have different research contribution and most of the papers contribute to generally one or more topics. This makes it hard to obtain ideal clustering.
\ei
Stating the above reasons, we do like to say that what we present is not the perfect modelling of the SE literature but a good approximation based on the 35k+ papers. The framework is open to extensions keeping the core topics like Source Code, Testing, Program Analysis and Requirements intact. For more details on this study we would like you to look into section \ref{sect:topicAdapt}.  \\

\textit{C.3. Regarding the interpretation of the results in section 4, the discussion of missing venues (RQ1), merging venues (RQ2) or growing/shrinking venues (RQ3) is too simplistic. Regarding RQ1, the issue of ``ICSM, CSRM, MSR, WCRE, ICPC'' not having a related journal might be due to different reasons. First of all, historically, less and less pure source code papers are published in these venues (and even in SCAM). Furthermore, most of the special issues of these conferences are published in EMSE, yet for some strange reason EMSE (and ESEM) are located relatively far from these conferences in Fig. 2's clusters.\\}

We agree, that was just silly in the last draft. We removed it.\\

\textit{C.4. Regarding RQ2, the statement that having too many venues is ``detrimental to the creation of new communities exploring newer ideas'' seems to be the other way around, since the more venues there are, the more space available for papers on even newer topics. Scarcity makes it more difficult to get a paper in, and hence to travel and meet the community. Furthermore, is there any evidence that the similar timing of ASE, ESEM and RE 2016 caused a problem for any of these three conferences in terms of number or quality of submissions, or amount of collaboration? The latter could be measured explicitly through analysis of the paper authors. A deeper question is to what extent do researchers pin themselves on one community rather than select the conference whose deadline is the closest? Similarly, the fact that ``the FSE workshops received very few submissions'' is a more common phenomenon that might not be due to ``SE researchers were so exhausted'' but rather that workshops have become less popular, since travelling is expensive and warrants a conference paper first. Furthermore, in order to propose merges between venues, one should also look at overlap between the authors publishing at different venues, and even though there is some overlap identified between venues, no pair has an entirely identical profile (see also my comment about considering citation count). As such, a deeper analysis is needed to really be able to claim that a merger would be useful.\\}


We agree! We were too silly. That content has been removed.\\

\textit{C.5. Fig. 4's anecdotal evidence does not really contribute much to the paper. Sure, as long as people review for multiple vendors, it is not possible to see their full review activities. Yet, this problem could be solved as well without merging the journals, as long as they start using the same review environments or DBs.\\}


Yes indeed. We've removed it.\\

\textit{C.6. Regarding RQ3, the identification of missing areas is rather ad hoc/anecdotal. Hence, basing funding and conference planning decisions on them is quite risky. The fact that a term like ``security'' or ``performance'' is not common in the analyzed venues seems more an issues caused by too low k, or by excluding niche conferences like ICPE from the study as well as systems conferences where security and performance are more common topics. In the latter case, recommending more mainstream venues to focus on these topics seems to introduce more overlap than it would resolve. The paper also does not consider special issues or conference paper extensions, which are two factors that could be responsible for overlap between journals and conferences.\\}

Thank you for your suggestions. The associate editor also agrees to this and considers this beyond the scope of this work. Hence, we removed these sections and now present this paper as a method to study trends in SE research.\\


\textit{C.7. Finally, I was concerned about the target audience of this paper. Except for newcomers to the field (junior or senior coming from other area), it is quite clear to researchers what is the scope/main topic of a venue based on the program of the last years. As such, I did not see many applications there. However, I do see usefulness for journals and conferences to find researchers working on the specific topic of a paper.\\}

We have listed some specific applications for this work-- see the four questions in the new Introduction(\tion{intro}).

That said, I think you'd agree that that this work has very broad application. The amazing thing about human text is that, when processed
in volume, it can exhibits fascinating regularities that can be used for a wide variety of tasks. No, we do not know the ultimate end user population of the methods of this page. But at a guess we would say that {\em many people} would be interested. \\


\textit{Page 1: `` What are the factors that prevent effective dissemination of research papers results? '':
It depends on what is meant by ``effective'', i.e., obtaining many citations, publishing in a venue with high impact factor, etc.}\\

You are right. In this paper we use citations and number of co-authored articles to define the term ``effective'' as shown in \tion{study_bias}. We note that in other work in progress, we expand this study to different impact factors like h-indices, harmonic mean of citations, page-rank etc. We think that there is another paper. As a courtesy to your interest we would like to show you those other results at \href{https://goo.gl/gcRBmp
}{goo.gl/gcRBmp}. Our view is that a analysis of what ``effective'' means is a complex issue, that requires  a separate paper. But please,  what is your view?\\

\textit{  Page 1: ``Different sets of topics that tend to be rejected from SE conferences or journals'':
As mentioned later as a threat to validity, the paper only studied accepted papers, hence the absence of certain topics does not necessarily mean that nobody is doing research in that area. Some topics might be notoriously reject-heavy.\\}

You are completely right. It is inappropriate for us to say that topics are rejected from different venues. What we can show is which papers are \underline{\textbf{accepted}} to different venues. Based on your comment we have replaced the inappropriate use of ``reject'' with ``accept''.
\\



\textit{  
Page 1: `` recent trend where SE conference papers are receiving significantly larger citations per year than journal papers.'':
This is not that recent, but well-known in the SE domain.\\}

We completely agree with you that, at this time there is an increasing emphasis on conference publications in SE. However, we are unaware of surveys of studies that provide evidence to that effect. One value added aspect of this work is that we can quantitatively define the size of that effect(\tion{study_conf_vs_jour}). \\

\textit{ Page 1: ``runs the risk of turning research into a ``game'' where authors deliberately distort their findings in order to increase the odds of getting papers accepted.'':
``distort'' as in falsifying data results, or as in writing a paper from a specific perspective to get in? The latter is commonplace even without the findings of this paper.\\} 

We agree with you comment. We have removed the reference to ``game''.\\

\textit{  Page 1: `` open-source toolkit that other researchers can apply together sets of documents:'':
Nice!\\} 

Thank you :-). \\

\textit{ Table 1: It is surprising how FSE/ASE are not grouped with ICSE, and that SANER is so similar to ICSE (and not to ICSME).\\}

You are right in this aspect that it is surprising that SANER is grouped close to ICSE. But, if you go up one level in the cluster hierarchy from \fref{div_heat}, you could see that all the generalist venues like ICSE, FSE, ASE, TSE and TOSEM are grouped in a single cluster along with ASE journal and SANER.\\

\textit{ Page 3: `` those conferences publications earn a significantly larger number of citations than journal articles'':
... yet in Table 1 journals like JSS and IST have a higher h-score?\\}

We would agree and disagree with you on that point. Venues like TSE, JSS, IST and IEEE software are top cited journals which lead to greater citations but when it comes to the rest of the journals, it leads to lesser number citations compared to conferences. This can also be verified by the h5-indices produced by google scholar(\href{https://goo.gl/ti7vd4
}{goo.gl/ti7vd4
}) where we see that only 4 of the top 20 are journals. \\

\textit{ Page 4: `` objective of DE is to maximize the Raw Score (<n) which is similar to the Jaccard Similarity'':
What is the insight behind this, i.e., why this score and why maximize it?\\}

This is a complex issue. For a full discussion we turn your kind attention to Agrawal \etal's work on it~\cite{agrawal2016wrong}. In summary, we can say here that, the scores above are maximized when clusters are most stable. An optimizer that explores this stability generates models that exhibits the desired properties we want; Specifically as we discussed above(C2), we show that our clusters are stable to incremental additions of new venues. \\


\textit{ Page 4: `` we found that optimal values in this domain are k, α $\&$ β are 11, 0.847 $\&$0.764 respectively. '':
Are the results impacted by the order of documents?\\}

You are quite correct to impact of order effects on these results. That is the whole point of the Agrawal \etal paper. They show that they can mitigate for order effects using LDA and DE. We reproduced that effect for the datasets explored in this study. We point your kind attention to \tion{ldade}.\\

\textit{ Fig. 2: Do the numbers add up to 100\% vertically?\\}

Yes they do. \\


\textit{ Page 6: `` While our LDADE reported many more topics than these top 11, those occur at diminishingly low frequencies'':
How is this possible given the choice of k=11?\\}

We performed sensitivity studies with increasing values of ``k''. We found that, at say k=20, that nearly half the topics consumed 95\% of the corpus and the rest was spread across a very small percentage of topics.\\


\textit{ Page 6: `` The empirical software engineering conference and journals are also grouped: see ESEM+ESE;'':
Why are these clustered on the left half of the figure, away from other (heavily empirical) conferences like MSR and ICSE?\\}

Conferences like MSR are focused with source code but venues like ESEM and ESE focus more on qualitative analysis. \\


\textit{ Page 9: `` Downward arrows denote topics of increasing popularity.; Upward arrows show topics of decreasing popularity. '':
It would be interesting to derive venue popularity based on the topic popularity.\\}

We quite take your point that the methods produced here could lead to any number of future interesting results. Indeed, that is the strength of this whole approach. That said, we ask your permission not to add this to the paper since we are pushing the page limit.
\\



\textit{ Page 10: ``This could result in one of the ``gaming'' tactics discussed in our introduction'':
I don't think this threat is real, since the paper does not consider acceptance rates, number of citations, etc.\\}

We agree and it is removed now. \\

\textit{ Page 11: `` fails to address how the citation trends have been varying between conferences and journals and if it attributes towards the increased number of publications in conferences over journals. '':
Was this done by this paper?\\}

Thank you for asking, we have clarified that and corrected our text in the related work.
\\

\textit{ Page 12: Section 7 just repeats what has been mentioned before, maybe it should be merged with the conclusion?\\}

Thank you. We have deleted this section based on your suggestions.

Thank you for such in-depth feedback. We have now added different case studies which answers different scenarios pointed out by you in section~\ref{sect:results}.

==> tex_naive_vs_tuned_lda.tex <==
\begin{figure}[!htpb]
\centering
\includegraphics[scale=0.45]{png_naive_vs_tuned_lda.png}
   \caption{What are the optimal number of topics to model SE? Log-Likelihood of perplexity for 2 to 50 topics. Perplexity is the probability of all the words in an untrained document given the topic model. From the figure, LDA-DE requires 11 topics and LDA requires 20 topics to model SE publications.}
   \label{fig:naive_vs_ldade}
\end{figure}

==> tex_topic_overlaps.tex <==
\begin{figure}[!htpb]
\centering
\includegraphics[scale=0.45]{png_topic_overlaps.png}
   \caption{How stable is LDADE compared to LDA? Percentage of common terms in the top 10 terms between two most similar topics on 20 random shuffles of the document using LDA and LDA-DE. From the figure a) The worst overlap between topics in LDADE is equal to the average overlap in LDA b) The worst overlap between topics in LDA is almost equal to random selection.}
   \label{fig:topic_overlaps}
\end{figure}
